Constrained Reinforcement Learning for Dynamic Material Handling

As one of the core parts of flexible manufacturing systems, material handling involves storage and transportation of materials between workstations with automated vehicles. The improvement in material handling can impulse the overall efficiency of the manufacturing system. However, the occurrence of dynamic events during the optimisation of task arrangements poses a challenge that requires adaptability and effectiveness. In this paper, we aim at the scheduling of automated guided vehicles for dynamic material handling. Motivated by some real-world scenarios, unknown new tasks and unexpected vehicle breakdowns are regarded as dynamic events in our problem. We formulate the problem as a constrained Markov decision process which takes into account tardiness and available vehicles as cumulative and instantaneous constraints, respectively. An adaptive constrained reinforcement learning algorithm that combines Lagrangian relaxation and invalid action masking, named RCPOM, is proposed to address the problem with two hybrid constraints. Moreover, a gym-like dynamic material handling simulator, named DMH-GYM, is developed and equipped with diverse problem instances, which can be used as benchmarks for dynamic material handling. Experimental results on the problem instances demonstrate the outstanding performance of our proposed approach compared with eight state-of-the-art constrained and non-constrained reinforcement learning algorithms, and widely used dispatching rules for material handling.

==> codes/ga.tex <==
\begin{algorithm}[!ht]
\caption{Genetic algorithm.}
\label{alg:ga}
\color{blue}
\begin{algorithmic}[1] %[1] enables line numbers
\Require  Generation $N$, population $\mu$
\Ensure $x_{best}$
\State Initialise population $I$
% \State Get invalid action $ia$ from $s$
% \State Set $m$ as negative Infinity
% \State Logits $l\leftarrow \pi_{\theta}(\cdot|s)$
% \State Get $l'$ by replacing $\pi_{\theta}(a'|s)$ with $-\infty$ where $a'$ is invalid action.
% \State $\pi'_{\theta}(\cdot|s) \leftarrow$ softmax($l'$)
% \State Sample $a \sim \pi'_{\theta}(\cdot|s)$

% \State \textbf{return} solution
\end{algorithmic}
\end{algorithm}

==> experiment_rules.tex <==
\section{Experiment}
\todo[inline]{comparing with dispatching rule, DQN by Hu, }
\todo[inline]{meta heuristic? needed to review}
\subsection{Case instance}
The max number of tasks in the instance is 40 and at most 6 tasks for each decision time. All tasks are generated randomly. Due time of a task is generated according to its travel time. Handling time follows $U(20,70)$. Interval of task release follows $N(60,50)$.
\todo[inline]{notation}
The delay time of $t$ is calculated by Eq.\ref{eq:delay}. If $delay(t)==0$, then task $t$ does not been delayed.
\begin{eqnarray}
delay(t) = \max((t.travel+t.wait-t.due),0) \label{eq:delay}
\end{eqnarray}
Closer inspection of the equation shows relations between dispatching rules. Formulations of these rules are presented as follows.
\begin{itemize}
    \item FCFS : $\mathop{\arg\min}\limits_t (t.tao)$
    \item STD : $\mathop{\arg\min}\limits_t (t.travel)$
    \item EDD : $\mathop{\arg\min}\limits_t (t.tao+t.due)$
    \item LWT : $\mathop{\arg\max}\limits_t (t.wait)$
    \item NVF : $\mathop{\arg\min}\limits_t (t.travel\_load)$
\end{itemize}
Surprisingly, these dispatching rules partially describe the Eq. \ref{eq:delay}. To mix these rules, we relax the Eq. \ref{eq:delay}. Four extra parameters are added for a better balance. The procedure is shown as follows.
\begin{eqnarray}
delay(t) &=& \max((t.travel+t.wait-t.due),0)  \label{eq:delay} \nonumber \\
&=& \max((t.travel+t.wait+t.tao-(t.tao+t.due)),0)   \nonumber \\
&Then,& \nonumber \\
delay_{r}(t) &=& \alpha*(t.travel_load)+\beta t.wait+\gamma t.tao-\delta(t.tao+t.due) \nonumber \\
\end{eqnarray}
\todo[inline]{formulation of the generation}
\subsection{Setting}
\subsection{Experiment on dispatching rules}
We test five dispatching rules including first come first served (FCFS), shorest travel distance (STD), earliest due date first (EDD), longest waiting time (LWT) and nearest vehicles first (NVF) as well as the mix policy on the instance. Deferential algorithm is used to optimise the mix policy with 6 population and 50 generations.


\input{tables/dispatchings/dispatching_0307}
\subsection{Result}

==> tables/instance_table/constraintP.tex <==
% \begin{table*}[b]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
%     \toprule

%     Policy &Instance.0 & Instance.1 & Instance.2 & Instance.3 & Instance.4 & Instance.5 & Instance.6 & Instance.7 \\
%         \midrule
% RCPO & 0.0 & 20.0 & 100.0 & 96.7 & 83.3 & 100.0 & 100.0 & 100.0\\
% IPO & 56.7 & 43.3 & 60.0 & 56.7 & 60.0 & 36.7 & 96.7 & 80.0\\
% \midrule
% L-SAC & 30.0 & 33.3 & 66.7 & 73.3 & 53.3 & 26.7 & 93.3 & 90.0\\
% L-PPO & 23.3 & 50.0 & 43.3 & 53.3 & 33.3 & 36.7 & 93.3 & 96.7\\
% \midrule
% SAC & 96.7 & 0.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & 100.0\\
% PPO & 46.7 & 60.0 & 56.7 & 50.0 & 66.7 & 26.7 & 100.0 & 83.3\\
% \midrule
% FCFS & 10.0 & 30.0 & 13.3 & 20.0 & 13.3 & 23.3 & 100.0 & 90.0\\
% EDD & 83.3 & 100.0 & 100.0 & 86.7 & 93.3 & 70.0 & 100.0 & 60.0\\
% NVF & 33.3 & 46.7 & 56.7 & 16.7 & 63.3 & 16.7 & 100.0 & 80.0\\
% STD & 0.0 & 50.0 & 43.3 & 86.7 & 60.0 & 40.0 & 73.3 & 73.3\\
% Random & 0.0 & 16.7 & 10.0 & 10.0 & 3.3 & 0.0 & 33.3 & 26.7\\
% \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:cp}
% \end{table*}




\begin{table*}[t]
    \centering
        \normalsize
        \caption{Constraint satisfaction percentage (\%) of policies on 16 instances.}
        \resizebox{\textwidth}{!}{

    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule

Instance &RCPO & RCPO-NS&IPO & L-SAC & L-PPO & SAC & PPO & FCFS & EDD & NVF & STD & Random \\
        \midrule
% Instance.0 & 0.0& 56.7& 30.0& 23.3& 96.7& 46.7& 10.0& 83.3& 33.3& 0.0& 0.0\\
% Instance.1 & 20.0& 43.3& 33.3& 50.0& 0.0& 60.0& 30.0& 100.0& 46.7& 50.0& 16.7\\
% Instance.2 & 100.0& 60.0& 66.7& 43.3& 0.0& 56.7& 13.3& 100.0& 56.7& 43.3& 10.0\\
% Instance.3 & 96.7& 56.7& 73.3& 53.3& 100.0& 50.0& 20.0& 86.7& 16.7& 86.7& 10.0\\
% Instance.4 & 83.3& 60.0& 53.3& 33.3& 100.0& 66.7& 13.3& 93.3& 63.3& 60.0& 3.3\\
% Instance.5 & 100.0& 36.7& 26.7& 36.7& 0.0& 26.7& 23.3& 70.0& 16.7& 40.0& 0.0\\
% Instance.6 & 100.0& 96.7& 93.3& 93.3& 100.0& 100.0& 100.0& 100.0& 100.0& 73.3& 33.3\\
% Instance.7 & 100.0& 80.0& 90.0& 96.7& 100.0& 83.3& 90.0& 60.0& 80.0& 73.3& 26.7\\
Instance01 & 0.0& 40.0& 56.7& 30.0& 23.3& \textbf{96.7}& 46.7& 10.0& 83.3& 33.3& 0.0& 0.0\\
Instance02 & 20.0& 56.7& 43.3& 33.3& 50.0& 0.0& 60.0& 30.0& \textbf{100.0}& 46.7& 50.0& 16.7\\
Instance03 & \textbf{100.0}& 66.7& 60.0& 66.7& 43.3& 0.0& 56.7& 13.3& \textbf{100.0}& 56.7& 43.3& 10.0\\
Instance04 & 96.7& 53.3& 56.7& 73.3& 53.3& \textbf{100.0}& 50.0& 20.0& 86.7& 16.7& 86.7& 10.0\\
Instance05 & 83.3& 33.3& 60.0& 53.3& 33.3& \textbf{100.0}& 66.7& 13.3& 93.3& 63.3& 60.0& 3.3\\
Instance06 & \textbf{100.0}& 26.7& 36.7& 26.7& 36.7& 0.0& 26.7& 23.3& 70.0& 16.7& 40.0& 0.0\\
Instance07 & \textbf{100.0}& 96.7& 96.7& 93.3& 93.3& \textbf{100.0}& \textbf{100.0}& \textbf{100.0}& \textbf{100.0}& \textbf{100.0}& 73.3& 33.3\\
Instance08 & \textbf{100.0}& 80.0& 80.0& 90.0& 96.7& \textbf{100.0}& 83.3& 90.0& 60.0& 80.0& 73.3& 26.7\\
\midrule
% Instance.8 & 0.0& 56.7& 20.0& 26.7& 96.7& 46.7& 3.3& 16.7& 66.7& 0.0& 0.0\\
% Instance.9 & 20.0& 43.3& 36.7& 50.0& 0.0& 60.0& 33.3& 86.7& 53.3& 50.0& 20.0\\
% Instance.10 & 100.0& 60.0& 70.0& 50.0& 0.0& 63.3& 13.3& 100.0& 56.7& 53.3& 6.7\\
% Instance.11 & 96.7& 56.7& 70.0& 53.3& 100.0& 46.7& 16.7& 86.7& 20.0& 73.3& 10.0\\
% Instance.12 & 100.0& 60.0& 66.7& 50.0& 100.0& 73.3& 13.3& 86.7& 90.0& 100.0& 6.7\\
% Instance.13 & 100.0& 36.7& 20.0& 36.7& 0.0& 30.0& 20.0& 86.7& 23.3& 26.7& 0.0\\
% Instance.14 & 80.0& 96.7& 96.7& 100.0& 100.0& 100.0& 100.0& 100.0& 100.0& 70.0& 36.7\\
% Instance.15 & 100.0& 80.0& 90.0& 96.7& 100.0& 83.3& 86.7& 23.3& 56.7& 70.0& 13.3\\
Instance09 & 0.0& 30.0& 56.7& 20.0& 26.7& \textbf{96.7}& 46.7& 3.3& 16.7& 66.7& 0.0& 0.0\\
Instance10 & 20.0& 56.7& 43.3& 36.7& 50.0& 0.0& 60.0& 33.3& \textbf{86.7}& 53.3& 50.0& 20.0\\
Instance11 & \textbf{100.0}& 66.7& 60.0& 70.0& 50.0& 0.0& 63.3& 13.3& 100.0& 56.7& 53.3& 6.7\\
Instance12 & 96.7& 50.0& 56.7& 70.0& 53.3& \textbf{100.0}& 46.7& 16.7& 86.7& 20.0& 73.3& 10.0\\
Instance13 & \textbf{100.0}& 46.7& 60.0& 66.7& 50.0& \textbf{100.0}& 73.3& 13.3& 86.7& 90.0& \textbf{100.0}& 6.7\\
Instance14 & \textbf{100.0}& 20.0& 36.7& 20.0& 36.7& 0.0& 30.0& 20.0& 86.7& 23.3& 26.7& 0.0\\
Instance15 & 80.0& 96.7& 96.7& 96.7& \textbf{100.0}& \textbf{100.0}& \textbf{100.0}& \textbf{100.0}& \textbf{100.0}& \textbf{100.0}& 70.0& 36.7\\
Instance16 & \textbf{100.0}& 80.0& 80.0& 90.0& 96.7& \textbf{100.0}& 83.3& 86.7& 23.3& 56.7& 70.0& 13.3\\
\bottomrule
    \end{tabular}
    }

    \label{tab:cp}
\end{table*}

==> tables/instance_table/rShape.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
Instance & RCPO-M & RCPO-noshape \\
\midrule
No.0 &  \textbf{1840.00} /\textbf{56.67}&  1891.93- /58.82$\approx$\\
No.1 &  \textbf{1908.37} /\textbf{48.16}&  1979.53- /51.60$\approx$\\
No.2 &  \textbf{1914.83} /\textbf{45.00}&  1931.10$\approx$ /46.85$\approx$\\
No.3 &  \textbf{1956.87} /\textbf{40.47}&  2003.90- /52.95-\\
No.4 &  \textbf{1852.50} /\textbf{21.29}&  2028.83- /58.11-\\
No.5 &  \textbf{1911.13} /\textbf{41.00}&  2028.93- /88.78-\\
No.6 &  \textbf{1927.00} /\textbf{8.40}&  1951.40- /15.21-\\
No.7 &  \textbf{1898.00} /\textbf{21.02}&  1951.00- /41.81-\\
\midrule
&-/-& 7/5\\
\bottomrule
    \end{tabular}
    \caption{Comparison between RCPO-M and one without reward sharping. ``+/$\approx$/-'' indicates the agent performs statistically better/similar/worse than RCPO-M agent. Bold number indicates the highest makespan and tardiness. The number of instance that RCPO-M is superior than RCPO-noshape is denoted in the last row.}
    \label{tab:comRS}
\end{table}

==> tables/instance_table/result.tex <==
% \begin{table*}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%     \toprule
%          \multirow{2}{*}{Instance}&\multicolumn{2}{c|}{SAC}& \multicolumn{2}{c|}{RCPO} & \multicolumn{2}{c|}{FCFS} & \multicolumn{2}{c|}{EDD}  & \multicolumn{2}{c|}{NVF} & \multicolumn{2}{c|}{STD}  &\multicolumn{2}{c}{Random} \\
%          & makespan & tardiness & makespan & tardiness& makespan & tardiness& makespan & tardiness& makespan & tardiness & makespan & tardiness\\
% \midrule

% No.0 &  \textbf{1798.43} &49.10&  1840.00 &56.67&  2081.10 &90.17&  1903.17 &\textbf{33.88}&  1876.47 &69.63&  1868.80 &66.60&  2098.70 &124.53\\
% No.1 &  1950.00 &68.93&  \textbf{1908.37} &48.16&  2084.47 &82.29&  1968.57 &\textbf{29.61}&  1958.43 &56.40&  1961.73 &49.18&  2113.77 &103.12\\
% No.2 &  1965.00 &53.37&  \textbf{1914.83} &45.00&  2014.73 &64.16&  1977.80 &\textbf{26.46}&  1946.70 &49.59&  1921.30 &51.67&  2091.20 &143.71\\
% No.3 &  2002.00 &\textbf{28.87}&  \textbf{1956.87} &40.47&  2136.67 &104.97&  1988.10 &32.83&  2040.60 &66.68&  1970.70 &35.59&  2135.07 &123.14\\
% No.4 &  1900.00 &26.63&  \textbf{1852.50} &\textbf{21.29}&  2194.57 &122.49&  1950.70 &33.70&  1933.87 &56.34&  1917.07 &41.43&  2149.27 &118.98\\
% No.5 &  2011.87 &71.26&  \textbf{1911.13} &\textbf{41.00}&  2123.50 &85.19&  2016.80 &46.82&  1953.40 &78.54&  1955.37 &62.72&  2159.10 &129.26\\
% No.6 &  \textbf{1927.00} &12.63&  1927.00 &\textbf{8.40}&  1927.93 &11.19&  1940.53 &12.13&  1996.50 &21.83&  1983.67 &30.43&  2083.03 &70.18\\
% No.7 &  1914.10 &\textbf{15.66}&  1898.00 &21.02&  1933.57 &27.35&  2020.80 &45.31&  1944.63 &35.47&  \textbf{1883.53} &35.05&  2067.83 &89.53\\
% \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}


% \begin{table*}[]
%     \centering
%     % \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \toprule
% Policy &No.0 & No.1 & No.2 & No.3 & No.4 & No.5 & No.6 & No.7 \\
% \midrule
% RCPO & 1840.0 (56.7) & \textbf{1908.4}  (48.2) & \textbf{1914.8}  (45.0) & \textbf{1956.9}  (40.5) & \textbf{1852.5}  (\textbf{21.3}) & \textbf{1911.1}  (\textbf{41.0}) & \textbf{1927.0}  (\textbf{8.4}) & 1898.0 (21.0)\\
% SAC & \textbf{1798.4}  (49.1) & 1950.0 (68.9) & 1965.0 (53.4) & 2002.0 (\textbf{28.9}) & 1900.0 (26.6) & 2011.9 (71.3) & 1927.0 (12.6) & 1914.1 (\textbf{15.7})\\
% FCFS & 2081.1 (90.2) & 2084.5 (82.3) & 2014.7 (64.2) & 2136.7 (105.0) & 2194.6 (122.5) & 2123.5 (85.2) & 1927.9 (11.2) & 1933.6 (27.4)\\
% EDD & 1903.2 (\textbf{33.9}) & 1968.6 (\textbf{29.6}) & 1977.8 (\textbf{26.5}) & 1988.1 (32.8) & 1950.7 (33.7) & 2016.8 (46.8) & 1940.5 (12.1) & 2020.8 (45.3)\\
% NVF & 1876.5 (69.6) & 1958.4 (56.4) & 1946.7 (49.6) & 2040.6 (66.7) & 1933.9 (56.3) & 1953.4 (78.5) & 1996.5 (21.8) & 1944.6 (35.5)\\
% STD & 1868.8 (66.6) & 1961.7 (49.2) & 1921.3 (51.7) & 1970.7 (35.6) & 1917.1 (41.4) & 1955.4 (62.7) & 1983.7 (30.4) & \textbf{1883.5}  (35.1)\\
% Random & 2098.7 (124.5) & 2113.8 (103.1) & 2091.2 (143.7) & 2135.1 (123.1) & 2149.3 (119.0) & 2159.1 (129.3) & 2083.0 (70.2) & 2067.8 (89.5)\\
% \bottomrule
%     \end{tabular}
    
%     \caption{Average makspan and tardiness (in the brackets) over 30 independent trails. Bold number indicates the highest makespan or tardiness. }
%     \label{tab:my_label}
% \end{table*}





% \begin{table*}[h]
%     \centering
%     % \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \toprule
% Policy &No.0 & No.1 & No.2 & No.3 & No.4 & No.5 & No.6 & No.7 \\
% \midrule
% RCPOM & 1840.0 (56.7) & \textbf{1908.4}  (48.2) & 1914.8 (45.0) & \textbf{1956.9}  (40.5) & \textbf{1852.5}  (\textbf{21.3}) & \textbf{1911.1}  (\textbf{41.0}) & \textbf{1927.0}  (\textbf{8.4}) & 1898.0 (21.0)\\
% IPO & 1860.5 (48.6) & 1933.5 (50.4) & 1924.9 (47.6) & 1979.1 (49.6) & 1951.1 (47.0) & 1951.5 (71.4) & 1977.0 (14.8) & 1943.0 (34.9)\\
% L-SAC & 1884.8 (60.3) & 1987.4 (57.2) & 1933.7 (44.0) & 1973.5 (42.2) & 1955.4 (44.7) & 1992.9 (68.5) & 1983.9 (19.8) & 1923.6 (32.8)\\
% L-PPO & 1872.1 (59.5) & 1963.5 (52.3) & \textbf{1910.3}  (49.7) & 1984.0 (49.7) & 1954.0 (55.5) & 1968.6 (75.6) & 1979.7 (18.9) & 1899.2 (32.6)\\
% SAC & \textbf{1798.4}  (49.1) & 1950.0 (68.9) & 1965.0 (53.4) & 2002.0 (\textbf{28.9}) & 1900.0 (26.6) & 2011.9 (71.3) & 1927.0 (12.6) & 1914.1 (\textbf{15.7})\\
% PPO & 1858.0 (52.3) & 1941.8 (49.9) & 1918.2 (44.3) & 1995.3 (55.6) & 1937.1 (47.6) & 1961.0 (82.0) & 1988.6 (14.6) & 1920.7 (35.6)\\
% FCFS & 2081.1 (90.2) & 2084.5 (82.3) & 2014.7 (64.2) & 2136.7 (105.0) & 2194.6 (122.5) & 2123.5 (85.2) & 1927.9 (11.2) & 1933.6 (27.4)\\
% EDD & 1903.2 (\textbf{33.9}) & 1968.6 (\textbf{29.6}) & 1977.8 (\textbf{26.5}) & 1988.1 (32.8) & 1950.7 (33.7) & 2016.8 (46.8) & 1940.5 (12.1) & 2020.8 (45.3)\\
% NVF & 1876.5 (69.6) & 1958.4 (56.4) & 1946.7 (49.6) & 2040.6 (66.7) & 1933.9 (56.3) & 1953.4 (78.5) & 1996.5 (21.8) & 1944.6 (35.5)\\
% STD & 1868.8 (66.6) & 1961.7 (49.2) & 1921.3 (51.7) & 1970.7 (35.6) & 1917.1 (41.4) & 1955.4 (62.7) & 1983.7 (30.4) & \textbf{1883.5}  (35.1)\\
% Random & 2098.7 (124.5) & 2113.8 (103.1) & 2091.2 (143.7) & 2135.1 (123.1) & 2149.3 (119.0) & 2159.1 (129.3) & 2083.0 (70.2) & 2067.8 (89.5)\\
% \bottomrule
%     \end{tabular}
    
%     \caption{Average makspan and tardiness (in the brackets) over 30 independent trails. Bold number indicates the highest makespan and tardiness. }
%     \label{tab:result}
% \end{table*}

% \begin{table*}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
% \toprule
% Policy &No.0 & No.1 & No.2 & No.3  \\
% \midrule
% RCPO & 1840.00 (56.67) & \textbf{1908.37}  (48.16) & \textbf{1914.83}  (45.00) & \textbf{1956.87}  (40.47)\\
% SAC & \textbf{1798.43}  (49.10) & 1950.00 (68.93) & 1965.00 (53.37) & 2002.00 (\textbf{28.87})\\
% FCFS & 2081.10 (90.17) & 2084.47 (82.29) & 2014.73 (64.16) & 2136.67 (104.97)\\
% EDD & 1903.17 (\textbf{33.88}) & 1968.57 (\textbf{29.61}) & 1977.80 (\textbf{26.46}) & 1988.10 (32.83)\\
% NVF & 1876.47 (69.63) & 1958.43 (56.40) & 1946.70 (49.59) & 2040.60 (66.68)\\
% STD & 1868.80 (66.60) & 1961.73 (49.18) & 1921.30 (51.67) & 1970.70 (35.59)\\
% Random & 2098.70 (124.53) & 2113.77 (103.12) & 2091.20 (143.71) & 2135.07 (123.14)\\
% \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}

\renewcommand{\arraystretch}{1}

\begin{table*}[t]
\normalsize
    \centering
        \caption{Average makespan and tardiness (in the brackets) over 30 independent trails. Bold number indicates the highest makespan and tardiness.``+/$\approx$/-'' indicates the agent performs statistically better/similar/worse than RCPO agent. The number of policies that RCPO is better than others in terms of makespan and tardiness on each instance is given in the bottom row. }
    \resizebox{\textwidth}{!}{
      \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
Policy &Instance01 & Instance02 & Instance03 & Instance04 & Instance05 & Instance06 & Instance07 & Instance08 \\
\midrule
RCPO & 1840.0/56.7 & \textbf{1908.4}/48.2 & 1914.8/45.0 & \textbf{1956.9}/40.5 & \textbf{1852.5}/\textbf{21.3} & \textbf{1911.1}/\textbf{41.0} & \textbf{1927.0}/\textbf{8.4} & 1898.0/21.0\\
RCPO-NS & 1891.9-/58.8$\approx$ & 1979.5-/51.6$\approx$ & 1931.1$\approx$/46.9$\approx$ & 2003.9-/53.0- & 2028.8-/58.1- & 2028.9-/88.8- & 1951.4-/15.2- & 1951.0-/41.8-\\
IPO & 1860.5-/48.6+ & 1933.5$\approx$/50.4$\approx$ & 1924.9$\approx$/47.6$\approx$ & 1979.1-/49.6$\approx$ & 1951.1-/47.0- & 1951.5-/71.4- & 1977.0-/14.8- & 1943.0-/34.9-\\
L-SAC & 1884.8-/60.3$\approx$ & 1987.4-/57.2- & 1933.7$\approx$/44.0$\approx$ & 1973.5$\approx$/42.2$\approx$ & 1955.4-/44.7- & 1992.9-/68.5- & 1983.9-/19.8- & 1923.6-/32.8-\\
L-PPO & 1872.1-/59.5$\approx$ & 1963.5-/52.3$\approx$ & \textbf{1910.3}$\approx$/49.7$\approx$ & 1984.0-/49.7- & 1954.0-/55.5- & 1968.6-/75.6- & 1979.7-/18.9- & 1899.2$\approx$/32.6-\\
SAC & \textbf{1798.4}+/49.1+ & 1950.0-/68.9- & 1965.0-/53.4- & 2002.0-/\textbf{28.9}+ & 1900.0-/26.6- & 2011.9-/71.3- & 1927.0$\approx$/12.6- & 1914.1-/\textbf{15.7}+\\
PPO & 1858.0$\approx$/52.3+ & 1941.8$\approx$/49.9$\approx$ & 1918.2$\approx$/44.3$\approx$ & 1995.3-/55.6- & 1937.1-/47.6- & 1961.0-/82.0- & 1988.6-/14.6- & 1920.7$\approx$/35.6-\\
\midrule
FCFS & 2081.1-/90.2- & 2084.5-/82.3- & 2014.7-/64.2- & 2136.7-/105.0- & 2194.6-/122.5- & 2123.5-/85.2- & 1927.9$\approx$/11.2- & 1933.6-/27.4$\approx$\\
EDD & 1903.2$\approx$/\textbf{33.9}+ & 1968.6-/\textbf{29.6}+ & 1977.8-/\textbf{26.5}+ & 1988.1-/32.8+ & 1950.7-/33.7- & 2016.8-/46.8- & 1940.5-/12.1- & 2020.8-/45.3$\approx$\\
NVF & 1876.5$\approx$/69.6$\approx$ & 1958.4-/56.4$\approx$ & 1946.7-/49.6$\approx$ & 2040.6-/66.7- & 1933.9-/56.3- & 1953.4-/78.5- & 1996.5-/21.8- & 1944.6-/35.5-\\
STD & 1868.8$\approx$/66.6$\approx$ & 1961.7-/49.2$\approx$ & 1921.3$\approx$/51.7- & 1970.7-/35.6+ & 1917.1-/41.4- & 1955.4-/62.7- & 1983.7-/30.4- & \textbf{1883.5}+/35.1-\\
Random & 2098.7-/124.5- & 2113.8-/103.1- & 2091.2-/143.7- & 2135.1-/123.1- & 2149.3-/119.0- & 2159.1-/129.3- & 2083.0-/70.2- & 2067.8-/89.5-\\
\midrule
$F_m$/$F_t$ & 6/2 &9/4 &5/4 &10/6 &11/11 &11/11 &9/11 &8/8 \\
% RCPO-M & 1840.0/56.7 & \textbf{1908.4}/48.2 & 1914.8/45.0 & \textbf{1956.9}/40.5 & \textbf{1852.5}/\textbf{21.3} & \textbf{1911.1}/\textbf{41.0} & \textbf{1927.0}/\textbf{8.4} & 1898.0/21.0\\
% IPO & 1860.5-/48.6+ & 1933.5$\approx$/50.4$\approx$ & 1924.9$\approx$/47.6$\approx$ & 1979.1-/49.6$\approx$ & 1951.1-/47.0- & 1951.5-/71.4- & 1977.0-/14.8- & 1943.0-/34.9-\\
% \midrule
% L-SAC & 1884.8-/60.3$\approx$ & 1987.4-/57.2- & 1933.7$\approx$/44.0$\approx$ & 1973.5$\approx$/42.2$\approx$ & 1955.4-/44.7- & 1992.9-/68.5- & 1983.9-/19.8- & 1923.6-/32.8-\\
% L-PPO & 1872.1-/59.5$\approx$ & 1963.5-/52.3$\approx$ & \textbf{1910.3}$\approx$/49.7$\approx$ & 1984.0-/49.7- & 1954.0-/55.5- & 1968.6-/75.6- & 1979.7-/18.9- & 1899.2$\approx$/32.6-\\
% \midrule
% SAC & \textbf{1798.4}+/49.1+ & 1950.0-/68.9- & 1965.0-/53.4- & 2002.0-/\textbf{28.9}+ & 1900.0-/26.6- & 2011.9-/71.3- & 1927.0$\approx$/12.6- & 1914.1-/\textbf{15.7}+\\
% PPO & 1858.0$\approx$/52.3+ & 1941.8$\approx$/49.9$\approx$ & 1918.2$\approx$/44.3$\approx$ & 1995.3-/55.6- & 1937.1-/47.6- & 1961.0-/82.0- & 1988.6-/14.6- & 1920.7$\approx$/35.6-\\
% \midrule
% FCFS & 2081.1-/90.2- & 2084.5-/82.3- & 2014.7-/64.2- & 2136.7-/105.0- & 2194.6-/122.5- & 2123.5-/85.2- & 1927.9$\approx$/11.2- & 1933.6-/27.4$\approx$\\
% EDD & 1903.2$\approx$/\textbf{33.9}+ & 1968.6-/\textbf{29.6}+ & 1977.8-/\textbf{26.5}+ & 1988.1-/32.8+ & 1950.7-/33.7- & 2016.8-/46.8- & 1940.5-/12.1- & 2020.8-/45.3$\approx$\\
% NVF & 1876.5$\approx$/69.6$\approx$ & 1958.4-/56.4$\approx$ & 1946.7-/49.6$\approx$ & 2040.6-/66.7- & 1933.9-/56.3- & 1953.4-/78.5- & 1996.5-/21.8- & 1944.6-/35.5-\\
% STD & 1868.8$\approx$/66.6$\approx$ & 1961.7-/49.2$\approx$ & 1921.3$\approx$/51.7- & 1970.7-/35.6+ & 1917.1-/41.4- & 1955.4-/62.7- & 1983.7-/30.4- & \textbf{1883.5}+/35.1-\\
% Random & 2098.7-/124.5- & 2113.8-/103.1- & 2091.2-/143.7- & 2135.1-/123.1- & 2149.3-/119.0- & 2159.1-/129.3- & 2083.0-/70.2- & 2067.8-/89.5-\\
% \midrule
% &5/2 &8/4 &5/4 &9/5 &10/10 &10/10 &8/10 &7/7 \\
\bottomrule
    \end{tabular}
    }

    \label{tab:result}
\end{table*}

==> tables/instance_table/unseenResult.tex <==

\begin{table*}[ht]
\normalsize
    \centering
        \caption{Average makespan and tardiness (in the brackets) over 30 independent trails. Bold number indicates the highest makespan and tardiness.``+/$\approx$/-'' indicates the agent performs statistically better/similar/worse than RCPO agent. The number of policies that RCPO is better than others in terms of makespan and tardiness on each instance is given in the bottom row. }
    \resizebox{\textwidth}{!}{
      \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
Policy & Instance09 & Instance10 & Instance11 & Instance12 & Instance13 & Instance14 & Instance15 & Instance16 \\
\midrule
% RCPO-M & 1840.0/57.1 & \textbf{1917.6}/49.4 & \textbf{1900.3}/45.8 & \textbf{1954.3}/38.8 & \textbf{1862.7}/\textbf{18.4} & \textbf{1914.1}/\textbf{41.8} & 1960.8/19.6 & 1896.4/\textbf{21.3}\\
% IPO & 1860.5-/\textbf{48.6}+ & 1933.5$\approx$/50.4$\approx$ & 1924.9-/47.6$\approx$ & 1979.1-/49.6- & 1951.1-/47.0- & 1951.5-/71.4- & 1977.0-/14.8+ & 1943.0-/34.9-\\
% \midrule
% L-SAC & 1892.3-/62.0$\approx$ & 1983.6-/56.9$\approx$ & 1933.1-/43.4+ & 1974.5-/43.0$\approx$ & 1954.4-/41.0- & 1999.4-/70.9- & 1981.5-/18.6+ & 1930.3-/34.8-\\
% L-PPO & 1877.5-/60.8$\approx$ & 1961.3-/52.6$\approx$ & 1905.8$\approx$/49.5$\approx$ & 1980.9-/49.8- & 1960.2-/50.1- & 1965.5-/78.5- & 1975.1-/18.2+ & 1901.5$\approx$/33.1-\\
% \midrule
% SAC & \textbf{1801.3}+/49.3+ & 1950.0-/69.1- & 1956.0-/56.8- & 2000.0-/\textbf{28.6}+ & 1904.0-/27.3- & 2015.1-/71.1- & \textbf{1930.0}+/12.6+ & 1987.0-/38.2-\\
% PPO & 1863.1-/53.5+ & 1941.8$\approx$/50.1$\approx$ & 1913.2$\approx$/44.1$\approx$ & 1986.3-/55.0- & 1927.4-/41.4- & 1965.5-/85.9- & 1990.1-/15.0+ & 1908.2$\approx$/35.4-\\
% \midrule
% FCFS & 2089.3-/92.5- & 2045.4-/75.7- & 1996.9-/67.6- & 2107.1-/95.2- & 2191.9-/121.7- & 2130.1-/89.9- & 1934.1$\approx$/11.1+ & 1946.8-/35.8-\\
% EDD & 1996.9-/107.7- & 1976.3-/\textbf{33.4}+ & 1978.7-/\textbf{22.0}+ & 1997.6-/36.9$\approx$ & 1962.1-/37.0- & 1993.5-/44.6- & 1934.8$\approx$/\textbf{11.0}+ & 2052.3-/69.4-\\
% NVF & 1847.5$\approx$/57.2- & 1958.8-/54.3$\approx$ & 1926.6$\approx$/51.8$\approx$ & 2021.7-/65.9- & 1939.2-/41.2- & 1975.5-/89.8- & 2003.5-/19.3+ & 1933.8-/40.9-\\
% STD & 1894.1-/72.5- & 1958.2$\approx$/49.7$\approx$ & 1923.1$\approx$/52.4- & 1985.2-/38.1$\approx$ & 1905.1-/31.4- & 1974.3-/71.9- & 1990.3$\approx$/33.0- & \textbf{1885.2}+/38.6-\\

% Random & 2132.7-/135.3- & 2100.9-/99.5- & 2076.2-/144.4- & 2097.5-/106.3- & 2144.1-/102.6- & 2142.9-/123.6- & 2101.3-/81.1- & 2055.1-/94.1-\\
% \midrule
% &8/5 &7/3 &6/4 &10/6 &10/10 &10/10 &6/2 &7/10 \\

RCPO & 1840.0/57.1 & \textbf{1917.6}/49.4 & \textbf{1900.3}/45.8 & \textbf{1954.3}/38.8 & \textbf{1862.7}/\textbf{18.4} & \textbf{1914.1}/\textbf{41.8} & 1960.8/19.6 & 1896.4/\textbf{21.3}\\
RCPO-NS & 1904.6-/60.2$\approx$ & 1985.4-/52.0$\approx$ & 1931.6-/47.3$\approx$ & 1995.6-/51.0- & 2009.1-/55.0- & 2034.9-/92.6- & 1956.6$\approx$/16.2+ & 1941.0$\approx$/40.3-\\
IPO & 1860.5-/\textbf{48.6}+ & 1933.5$\approx$/50.4$\approx$ & 1924.9-/47.6$\approx$ & 1979.1-/49.6- & 1951.1-/47.0- & 1951.5-/71.4- & 1977.0-/14.8+ & 1943.0-/34.9-\\
L-SAC & 1892.3-/62.0$\approx$ & 1983.6-/56.9$\approx$ & 1933.1-/43.4+ & 1974.5-/43.0$\approx$ & 1954.4-/41.0- & 1999.4-/70.9- & 1981.5-/18.6+ & 1930.3-/34.8-\\
L-PPO & 1877.5-/60.8$\approx$ & 1961.3-/52.6$\approx$ & 1905.8$\approx$/49.5$\approx$ & 1980.9-/49.8- & 1960.2-/50.1- & 1965.5-/78.5- & 1975.1-/18.2+ & 1901.5$\approx$/33.1-\\
SAC & \textbf{1801.3}+/49.3+ & 1950.0-/69.1- & 1956.0-/56.8- & 2000.0-/\textbf{28.6}+ & 1904.0-/27.3- & 2015.1-/71.1- & \textbf{1930.0}+/12.6+ & 1987.0-/38.2-\\
PPO & 1863.1-/53.5+ & 1941.8$\approx$/50.1$\approx$ & 1913.2$\approx$/44.1$\approx$ & 1986.3-/55.0- & 1927.4-/41.4- & 1965.5-/85.9- & 1990.1-/15.0+ & 1908.2$\approx$/35.4-\\
\midrule
FCFS & 2089.3-/92.5- & 2045.4-/75.7- & 1996.9-/67.6- & 2107.1-/95.2- & 2191.9-/121.7- & 2130.1-/89.9- & 1934.1$\approx$/11.1+ & 1946.8-/35.8-\\
EDD & 1996.9-/107.7- & 1976.3-/\textbf{33.4}+ & 1978.7-/\textbf{22.0}+ & 1997.6-/36.9$\approx$ & 1962.1-/37.0- & 1993.5-/44.6- & 1934.8$\approx$/\textbf{11.0}+ & 2052.3-/69.4-\\
NVF & 1847.5$\approx$/57.2- & 1958.8-/54.3$\approx$ & 1926.6$\approx$/51.8$\approx$ & 2021.7-/65.9- & 1939.2-/41.2- & 1975.5-/89.8- & 2003.5-/19.3+ & 1933.8-/40.9-\\
STD & 1894.1-/72.5- & 1958.2$\approx$/49.7$\approx$ & 1923.1$\approx$/52.4- & 1985.2-/38.1$\approx$ & 1905.1-/31.4- & 1974.3-/71.9- & 1990.3$\approx$/33.0- & \textbf{1885.2}+/38.6-\\
Random & 2132.7-/135.3- & 2100.9-/99.5- & 2076.2-/144.4- & 2097.5-/106.3- & 2144.1-/102.6- & 2142.9-/123.6- & 2101.3-/81.1- & 2055.1-/94.1-\\
\midrule
$F_m$/$F_t$ &9/5 &8/3 &7/4 &11/7 &11/11 &11/11 &6/2 &7/11 \\


\bottomrule
    \end{tabular}
    }

    \label{tab:unseenResult}
\end{table*}
